Exchangeable Random Measures for Sparse and Modular Graphs with Overlapping Communities

We propose a novel statistical model for sparse networks with overlapping community structure. The model is based on representing the graph as an exchangeable point process, and naturally generalizes existing probabilistic models with overlapping block-structure to the sparse regime. Our construction builds on vectors of completely random measures, and has interpretable parameters, each node being assigned a vector representing its level of affiliation to some latent communities. We develop methods for simulating this class of random graphs, as well as to perform posterior inference. We show that the proposed approach can recover interpretable structure from two real-world networks and can handle graphs with thousands of nodes and tens of thousands of edges.

==> figures/tikz3.tex <==
\begin{tikzpicture}[node distance=1.4cm, auto,>=latex',scale=.8]
\draw[->,ultra thick] node[left] {0} (0,0) -- (6,0) node[right] {};
\draw[->,ultra thick] (0,0) -- (0,-6) node[right] {};
\draw[fill=blue,opacity=0.1] (0,0) -- (0,-6) -- (6,-6) -- (6,0)  ;
% Draw the grid
\draw[dashed] (1,1.5) -- (1,-1) node[right] {};
\draw[dashed] (3,2.5) -- (3,-3) node[right] {};
\draw[dashed] (3.5,3) -- (3.5,-3.5) node[right] {};
\draw[dashed] (5,4.5) -- (5,-5) node[right] {};
\draw[dashed] (0,-1) -- (1,-1) node[right] {};
\draw[dashed] (0,-3) -- (3,-3) node[right] {};
\draw[dashed] (0,-3.5) -- (3.5,-3.5) node[right] {};
\draw[dashed] (0,-5) -- (5,-5) node[right] {};
\node at (-.3,1) {0};
%\node at (-.3,1.5) {1};
\node at (-.3,2) {2};
%\node at (-.3,2.5) {3};
\node at (-.3,3) {4};
%\node at (-.3,3.5) {5};
\node at (-.3,4) {6};
\node at (6,.5) {$\alpha$};
%\node at (-.3,4.5) {7};
\draw[-,ultra thick,blue] (1,4.5) -- (1.5,4.5) node[right] {$\color{blue} N_\alpha$};
\draw[-,ultra thick,red] (1,4) -- (1.5,4) node[right] {$\color{red} N_\alpha^{(e)}$};
% draw the point process
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (1,-1) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (1,-5) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (3,-1.5) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (3.5,-1) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (5,-1) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (1.5,-3) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (1,-3.5) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (5,-3.5) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (3.5,-5) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (5,-0.5) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (0.5,-5) {};
\node[draw,circle,inner sep=2.5pt,fill=blue,shading=ball] at (5,-5) {};


\draw[->,ultra thick] node[left] {0} (0,1) -- (6,1) node[right] {};
\draw[->,ultra thick] (0,1) -- (0,5) node[right] {};
\draw[-,ultra thick,blue] (0,1.05) -- (1,1.05) node[right] {};
\draw[-,ultra thick,blue] (1,1.55) -- (3,1.55) node[right] {};
\draw[-,ultra thick,blue] (3,2.5) -- (3.5,2.5) node[right] {};
%\draw[-,ultra thick,blue] (3,3) -- (3.5,3) node[right] {};
\draw[-,ultra thick,blue] (3.5,3) -- (5,3) node[right] {};
\draw[-,ultra thick,blue] (5,3.5) -- (5.5,3.5) node[right] {};

\draw[-,ultra thick,red] (0,1) -- (1,1) node[right] {};
\draw[-,ultra thick,red] (1,1.5) -- (3,1.5) node[right] {};
\draw[-,ultra thick,red] (3,2) -- (3.5,2) node[right] {};
\draw[-,ultra thick,red] (3,2) -- (3.5,2) node[right] {};
\draw[-,ultra thick,red] (3.5,2.5) -- (5,2.5) node[right] {};
\draw[-,ultra thick,red] (5,4.5) -- (5.5,4.5) node[right] {};
%\node[] at (5.4,-3.8) {$\color{blue}z_{ij}$};
%\node[red] at (5,-.3) {$\color{red}\theta_{i}$};
%\node[red] at (.3,-3.5) {$\color{red}\theta_{j}$};
% Draw the increments of the Lévy process
%\draw[-,ultra thick,red] (1,0) -- (1,1) node[right] {};
%\draw[-,ultra thick,red] (3,0) -- (3,.3) node[right] {};
%\draw[-,ultra thick,red] (3.5,0) -- (3.5,.35) node[right] {};
%\draw[-,ultra thick,red] (5,0) -- (5,.5) node[above] {$\color{red}w_i$};
%\draw[-,ultra thick,red] (.6,0) -- (.6,.2) node[right] {};
%\draw[-,ultra thick,red] (1.2,0) -- (1.2,.1) node[right] {};
%\draw[-,ultra thick,red] (4.1,0) -- (4.1,.2) node[above] {};
%\draw[-,ultra thick,red] (0, -1) -- (-1,-1) node[right] {};
%\draw[-,ultra thick,red] (0,-3) -- (-.3,-3) node[right] {};
%\draw[-,ultra thick,red] (0,-3.5) -- (-.35,-3.5) node[left] {$\color{red}w_j$};
%\draw[-,ultra thick,red] (0,-5) -- (-.5,-5) node[right] {};
%\draw[-,ultra thick,red] (0,-.6) -- (-.2,-.6) node[right] {};
%\draw[-,ultra thick,red] (0,-1.2) -- (-.1,-1.2) node[right] {};
%\draw[-,ultra thick,red] (0,-4.1) -- (-.2,-4.1) node[right] {};
\end{tikzpicture}


